Learning to Search in Task and Motion Planning with Streams

Task and motion planning problems in robotics combine symbolic planning over discrete task variables with motion optimization over continuous state and action variables. Recent works such as PDDLStream have focused on optimistic planning with an incrementally growing set of objects until a feasible trajectory is found. However, this set is exhaustively expanded in a breadth-first manner, regardless of the logical and geometric structure of the problem at hand, which makes long-horizon reasoning with large numbers of objects prohibitively time-consuming. To address this issue, we propose a geometrically informed symbolic planner that expands the set of objects and facts in a best-first manner, prioritized by a Graph Neural Network that is learned from prior search computations. We evaluate our approach on a diverse set of problems and demonstrate an improved ability to plan in difficult scenarios. We also apply our algorithm on a 7DOF robotic arm in block-stacking manipulation tasks.

==> old.tex <==
% Task and motion planning (TAMP) involves planning high-level symbolic actions and corresponding low level controls, while accounting for geometric considerations \cite{garrett2020integrated}. 
% As a motivating example, consider the block-rearrangement task for a robot arm in Figure \ref{fig:2D_panda}. We must plan both with the actions move, pick, place etc., while specifying a collision-free trajectory for the robotic arm. Planning purely symbolically would result in trying to grasp \texttt{b0} first, causing a collision with \texttt{b2}. 
%Many TAMP problems are currently intractable with state-of-the-art techniques. For sampling-based TAMP algorithms, this difficulty stems from the rapid expansion of the number of symbolic objects and facts in the planning problems. This is because an infinite space of continuous valued quantities must be discretized. For example, for each block in Figure \ref{fig:2D_panda}, there are infinitely many valid grasp poses and placement poses, and collision-free trajectories between those poses, supporting infinitely many potential actions.

% PDDLStream is an open-source, domain independent, TAMP framework \cite{garrett2020pddlstream}. ...

% our contributions:
% We present a learning-based, probabilistic complete, extension to PDDLStream, turning the search in the space of streams instances from breadth first to "best-first".

% What problem are we solving:

% What is TAMP?
% introduce motivating example to explain (Figure 1)
% Explain a PDDLStream, and why the SOTA methods suffer from an explosion of stream results
% Explain the core idea behind our algorithm, and why it will help

% Proof:
% Comparison between ADAPTIVE, FOCUSED (two state of the art PDDLStream algorithms) and INFORMED (ours) across 3 domains:
% kitchen
% blocks world (with 5 subdomains)
% hanoi
% We demonstrate that INFORMED outpreformes ADAPTIVE and FOCUSED on all domains. 
% Finally, we show sim-to-real transfer of this technique on a real Franka-Panda robot arm.

